Designing an Adaptive Application-Level Checkpoint Management System for Malleable MPI Applications

Dynamic resource management opens up numerous opportunities in High Performance Computing. It improves the system-level services as well as application performance. Checkpointing can also be deemed as a system-level service and can reap the benefits offered by dynamism. A checkpointing system can have better resource availability by integrating with a malleable resource management system. In addition to fault tolerance, the checkpointing system can cater to the data redistribution demand of malleable applications during resource change. Therefore, we propose iCheck, an adaptive application-level checkpoint management system that can efficiently utilize the system and application level dynamism to provide better checkpointing and data redistribution services to applications.

==> sections/background.tex <==
\section{Malleable Infrastructure}
\label{sec:bg}

We have used the malleable infrastructure from the InvasiC project\cite{compres17,chadhaextend} as a test bed for our investigation into designing a malleable checkpointing system. It consists of an MPI implementation that can change the number of processes during the application execution and a malleable research manager that can orchestrate the resource changes in MPI. Malleable MPI, an extension of MPICH, adds four additional methods to standard MPI to bring resource dynamism (See Listing Listing \ref{icheckapi}). The malleable resource manager consists of a fork of the Slurm \cite{yoo2003slurm} and extensions to support resource-aware applications. %\texttt{MPI\_Init\_adapt} initialises a malleable application. \texttt{MPI\_Probe\_adapt} checks for a resource change. \texttt{MPI\_Comm\_adapt\_begin} starts the resource change and \texttt{MPI\_Comm\_adapt\_commit} finalises the resource change.
% \begin{itemize}
%     \item \texttt{MPI\_INIT\_ADAPT}: Initialises a malleable application
%     \item \texttt{MPI\_PROBE\_ADAPT}: Checks for a resource change
%     \item \texttt{MPI\_COMM\_ADAPT\_BEGIN}: Starts the resource change
%     \item \texttt{MPI\_COMM\_ADAPT\_COMMIT}: Finalises the resource change
% \end{itemize}

==> sections/evaluation.tex <==
\section{Experimental evaluation}
\label{sec:eval}
%This section analyses the performance of iCheck, overhead induced by iCheck, and the effect of different agent distribution and agent placement strategies on checkpointing.

%\begin{figure*}[t]
%    \centering
%    \begin{subfigure}{0.46\textwidth}
%    \centering
%        \includegraphics[width=0.86\linewidth]{images/ic_ls_agent_log.png}
%        \caption{Comparing iCheck and MPI-IO with different agents}
%        \label{fig:ic_blk_mpiio_agents}
%    \end{subfigure}
%    \begin{subfigure}{0.46\textwidth}
%    \centering
%        \includegraphics[width=0.86\linewidth]{images/ic_ls_blk_mpiio_nodes.png}
%        \caption{Comparing iCheck and MPI-IO with different nodes}
%        \label{fig:ic_blk_mpiio_nodes}    
%    \end{subfigure}
    
%    \begin{subfigure}{0.46\textwidth}
%    \centering
%        \includegraphics[width=0.86\linewidth]{images/ic_ls_blk_nonblk.png}
%        \caption{Comparing blocking vs non-blocking strategies in iCheck}
%        \label{fig:ic_blk_nblk_comparison}
%    \end{subfigure}
%    \begin{subfigure}{0.46\textwidth}
%    \centering
%        \includegraphics[width=0.86\linewidth]{images/ic_ls_pull_push.png}
%        \caption{Comparing push and pull strategies}
%        \label{fig:ic_push_pull}
%    \end{subfigure}
%    \caption{Checkpointing analysis on ls1 mardyn using iCheck and MPI-IO}
%    \label{fig_0}
%\end{figure*}
\subsection{Evaluation Setup}
\subsubsection{System}
The evaluation of iCheck is performed on the high performance system SuperMUC-NG~\cite{supermuc} at Leibniz Supercomputing Centre in Germany. A compute node consists of 2 Intel Xeon 8174 processors, with 96 GB DDR4 Memory with Intel OmniPath Adapter and Gigabit Ethernet adapter. Intel OmniPath Interconnect~\cite{Birrittella2015IntelOA} network with fat-tree network topology provides a high bandwidth networking between compute nodes. The parallel file system features 500 Gbytes of I/O bandwidth for the HPC system. Sixteen nodes (768 cores) were used for our evaluation, in which iCheck used up to four nodes, and applications were launched in the remaining nodes based on the evaluation objective.
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.46\textwidth}
    \centering
        \includegraphics[width=0.86\linewidth]{images/ic_ls1overhead.png}
        \caption{Total overhead of checkpointing}
        \label{fig:ic_ls1_overhead}
    \end{subfigure}
    \begin{subfigure}{0.46\textwidth}
    \centering
        \includegraphics[width=0.86\linewidth]{images/ic_ls_node_ds.png}
        \caption{Breakdown of iCheck induced overhead}
        \label{fig:ic_ls1_node_overhead}    
    \end{subfigure}
    \caption{Overhead comparison of iCheck and MPI-IO on ls1 mardyn}
    \label{fig_1}
\end{figure*}

%\begin{figure*}[t]
%    \centering
%    \begin{subfigure}{0.46\textwidth}
%    \centering
%        \includegraphics[width=0.86\linewidth]{images/ic_synth_icheck_mpiio_12_scr.png}
%        \caption{Comparing iCheck, MPI-IO and SCR on checkpointing large data size}
%        \label{fig:ic_synthetic_cp_compare}
%    \end{subfigure}
%    \begin{subfigure}{0.46\textwidth}
%    \centering
%        \includegraphics[width=0.86\linewidth]{images/ic_synth_overhead_12.png}
%        \caption{Overhead analysis of various iCheck operations}
%        \label{fig:ic_synth_overhead}
%    \end{subfigure}
%    \caption{Checkpointing analysis on synthetic application using iCheck and MPIIO}
%    \label{fig:synth_icheck_mpiio}
%\end{figure*}
\subsubsection{Applications}
The iCheck system is assessed with a highly scalable molecular dynamics application ls1 mardyn~\cite{doi:10.1021/ct500169q}, hydrodynamics proxy application LULESH~\cite{LULESH2}, Jacobi 2D heat simulation code, and a synthetic benchmark application that checkpoints the specified size in intervals and duration provided by the user.
%We have added iCheck support to ls1 mardyn, LULESH, Jacobi and created a synthetic benchmark as part of the evaluation process. The ls1 mardyn has an in-house checkpointing using MPI-IO implementation, and we compare iCheck against this implementation. We perform extensive iCheck library overhead analysis, dynamic agent evaluations, and comparison with MPI-IO in the ls1 mardyn and synthetic benchmark application. LULESH and the heat simulation application was used along with ls1 mardyn and synthetic application to demonstrate the dynamism in iCheck. The ls1 mardyn has an in-house checkpointing using MPI-IO implementation, and we compare iCheck against this implementation. 
We launched ls1 mardyn application on one (48 processes) to twelve (576 processes) nodes for the analysis. For data transfer tests (Subsections \ref{subsec:ls1},\ref{subsec:ls1_blk_nblk} and \ref{subsec:ls1_pp}), we ran ls1 mardyn for 100 time steps with a checkpoint interval of ten time steps. These quick runs were also used to stress test the iCheck infrastructure. For overhead analysis (Subsection \ref{subsec:overheads_library}), we ran ls1 mardyn for 10000 time steps, in which iCheck and MPI-IO checkpoints every 1000 time steps. The simulation system was initialized with 65536 molecules and checkpointed eight megabytes during each checkpoint operation for all the tests. Each of the process stores information about molecules like id, position, momentum, velocity, etc. The synthetic application was also run on one to twelve nodes (48 to 576 processes) by writing a checkpoint of size up to 2.3 GB per checkpoint operation. LULESH was run on two nodes and the heat simulation application was run on two to twelve nodes to study the malleability of iCheck.
%\subsubsection{Test Scenario}
%We ran ls1 mardyn application on one (48 processes) to twelve (576 processes) nodes. For data transfer tests (comparison with MPI-IO, blocking and non-blocking, push and pull techniques), we ran ls1 mardyn for 100 time steps with a checkpoint interval in ten time steps. These quick runs were also used to stress test the iCheck infrastructure. For overhead analysis, we ran ls1 mardyn for 10000 time steps, in which iCheck and MPI-IO checkpoints every 1000 time steps. For all the tests, the simulation system was initialized with 65536 molecules. Each of the process stores information about molecules like id, position, momentum, velocity, etc. %The synthetic application was also run on one to twelve nodes (48 to 576 processes) by writing a checkpoint of size up to 2.3 GB per checkpoint operation. LULESH was run on two nodes and the heat simulation application was run on two to twelve nodes to study the malleability of iCheck.
\subsection{Results} \label{subsec:results}
%\subsubsection{iCheck vs MPI-IO in ls1 mardyn} \label{subsec:ls1}
%In the following analysis, the blocking checkpointing strategy of iCheck is compared with the in-house MPI-IO based checkpointing provided by ls1 mardyn. Figure \ref{fig:ic_blk_mpiio_agents} (in log scale) and \ref{fig:ic_blk_mpiio_nodes} depict the average time taken for a checkpoint transfer operation performed by iCheck and MPI-IO during the execution of ls1 mardyn. Figure \ref{fig:ic_blk_mpiio_agents} shows the time taken by iCheck with agents varying from one to twelve and MPI-IO during the application run on twelve nodes, while Figure \ref{fig:ic_blk_mpiio_nodes} plots the iCheck and MPI-IO time while running the application on one, four, eight and twelve nodes with a single agent inside a single iCheck node.

%It can be observed from both the figures that the iCheck performs better than MPI-IO versions in all the configurations. A comparison with the worst-performing single iCheck agent with the MPI-IO in Figure \ref{fig:ic_blk_mpiio_agents} shows that iCheck is around 400 times faster in writing checkpoints than MPI-IO. The best iCheck configuration with 12 agents performs around 5000 times faster than MPI-IO. Similarly, the same trend is observable in Figure \ref{fig:ic_blk_mpiio_nodes}, with iCheck taking .8 to 1 millisecond, while MPI-IO ranges from 100 to 700 milliseconds. Another observation from Figure \ref{fig:ic_blk_mpiio_nodes} is that as the application's nodes increase, the checkpointing time by iCheck increases if there are no changes in the number of agents.

\subsubsection{Blocking vs Non-Blocking checkpointing in ls1 mardyn} \label{subsec:ls1_blk_nblk}
%Here, we show the difference between blocking and non-blocking checkpoint transfers of iCheck in ls1 mardyn (see Figure \ref{fig:ic_blk_nblk_comparison}). It compares the performance delivered by different agent configurations. It can be deduced from Figure \ref{fig:ic_blk_nblk_comparison} that the non-blocking mode of iCheck yields better performance than the blocking mode in every agent configuration. The non-blocking agent combinations perform up to 50\% faster than the blocking combinations. Furthermore, we can observe that the non-blocking version provides the combined performance of the blocking version plus the improvement gained by an additional agent. Another insight from the graph is that as the number of agents increases, the checkpoint transfer happens more quickly in blocking and non-blocking combinations.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.35\textwidth]{images/ic_synthetic.png}
%     \caption{Analysing different phases of checkpointing in iCheck}
%     \label{fig:ic_synthetic}
% \end{figure}
%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=0.35\textwidth]{images/ic_ls1overhead.png}
%    \caption{Overhead comparison of iCheck and MPIIO on ls1 mardyn}
%    \label{fig:ic_ls1_overhead}
%\end{figure}

%\begin{figure*}[t]
%    \centering
%    \begin{subfigure}{0.46\textwidth}
%    \centering
%        \includegraphics[width=0.86\linewidth]{images/ic_heat_dyn.png}
%        \caption{Impact of dynamic agent adaptation on a 2D heat simulation}
%        \label{fig:ic_heat_dyn}
%    \end{subfigure}
%    \begin{subfigure}{0.46\textwidth}
%    \centering
%        \includegraphics[width=0.86\linewidth]{images/ic_synth_agent_placement.png}
%        \caption{Effect of agent placement strategies on synthetic application}
%        \label{fig:ic_synthetic_distribution}
%    \end{subfigure}
%    \caption{Effect of dynamic agents and agent placement strategies}
%    \label{fig:ic_agent_placement}
%\end{figure*}
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.46\textwidth}
    \centering
        \includegraphics[width=0.86\linewidth]{images/ic_hs_mc.png}
        \caption{Number of active iCheck nodes in the system}
        \label{fig:ic_scale}
    \end{subfigure}
    \begin{subfigure}{0.46\textwidth}
    \centering
        \includegraphics[width=0.86\linewidth]{images/ic_hs_ag_mg_ds.png}
        \caption{Distribution of agents across iCheck nodes}
        \label{fig:ic_scale_dist}
    \end{subfigure}
    \caption{Demonstrating the horizontal scaling in iCheck during a time interval}
    \label{fig_dynamic}
\end{figure*}
\subsubsection{Push vs Pull strategies in ls1 mardyn}\label{subsec:ls1_pp}

%Figure~\ref{fig:ic_push_pull} compares the push and pull strategies mentioned in Section \ref{using_rdma}. We can observe from the graph that the push strategy performs better than the pull strategy. In ls1 mardyn, each process has a different number of molecules, which changes during the application execution. Hence, the agents must read the new checkpoint size before transferring the checkpoint and induces an additional overhead in pull strategy. With a single agent, the push strategy is 40\% faster than the pull strategy, and this can be attributed to the fact that a single agent needs to read the checkpoint size before transferring the checkpoint from all the application nodes. As we increase the number of agents, the advantage provided by the push strategy is barely visible. Hence, we can conclude that the push strategy is ideal for single-agent applications. %Since iCheck supports non-MPI applications, this strategy can be set as the default option for non-MPI applications. 

\subsubsection{iCheck overhead analysis in ls1 mardyn} \label{subsec:overheads_library}

%In this subsection, we show the overhead induced by iCheck on ls1 mardyn (See Figure \ref{fig:ic_ls1_overhead} (in log scale)). The application was run for 10000 time steps with checkpointing performed every 1000 steps. The overhead induced by iCheck on ls1 mardyn can be analyzed from two aspects. The first aspect explores the overall impact of iCheck and MPI-IO on the application run (See Figure~\ref{fig:ic_ls1_overhead}).We can infer that the total time spent on iCheck calls is only .03\% of the total application time, while MPI-IO took around 5.6\%. A significant portion of overhead comes from the initial setup of iCheck. The overall checkpoint performance of the iCheck library improves as the application progresses, which can be attributed to the iCheck commit operation that takes only a minuscule time to transfer checkpoints compared to MPI-IO. Furthermore, ls1 mardyn has six percentage faster execution with a single iCheck agent.

%To analyze the impact of the iCheck initial setup, we ran ls1 mardyn on one, four, eight, and twelve nodes (See Figure~\ref{fig:ic_ls1_node_overhead} (in log scale)). A single agent, which delivers the poorest performance in iCheck (as seen in Figure~\ref{fig:ic_blk_mpiio_agents}), is used for comparison with MPI-IO. We can observe that as the number of processes increases, configuration time in iCheck increases. A similar trend is visible for all operations plotted in the graph, including time taken for MPI-IO. Furthermore, we can observe that the first checkpoint transfer needed additional time than subsequent checkpoint transfers %(See the time taken for the remaining checkpoints in Figure~\ref{fig:ic_blk_mpiio_agents}). 
%This is for the libfabric memory region registration and shared memory configuration performed inside the library and agents. Another interesting observation from the figure is that the total time taken by iCheck for initialization and first checkpoint transfer is comparable to a single checkpoint transfer using MPI-IO. From the second commit onwards, iCheck starts outperforming MPI-IO. Nevertheless, the configuration time in iCheck can be reduced significantly by using more agents. %and is depicted in the next subsection.

\subsubsection{Comparing iCheck with SCR and MPI-IO using a synthetic application} \label{subsec:synth}
%In this subsection, we first compare the performance of iCheck against MPI-IO and state-of-the-art Scalable Checkpoint/Restart~\cite{scr} using a synthetic application. In this analysis, the application was run on 12 nodes (576 processes) and checkpointed 2.3 GB of data. Further, we discuss the overhead induced by iCheck on large checkpoint transfers. %We also analyse the effect of different agent placement strategies (see section  ~\ref{sec:iCheck}) on data transfer. 

%Figure~\ref{fig:ic_synthetic_cp_compare} depicts the average time for checkpoint transfer in iCheck and MPI-IO.  We can observe from the figure that iCheck performs 3.9 times faster than SCR and 7.6 times faster than MPI-IO while using a single agent. As we increase the number of agents, iCheck provides up to 57 and 100 times faster data transfer than SCR and MPI-IO, respectively. 

%Figure \ref{fig:ic_synth_overhead} shows the agent creation time or initialization time (\verb|icheck_init|), checkpoint data transfer time (\verb|icheck_commit|), finalization time (\verb|icheck_finalize|) and the time taken to restore (\verb|icheck_restart|) the checkpointed data for up to twelve agents. We can observe in the figure that increase in agents can reduce the iCheck induced overhead on the application. The contrast in performance between restart and commit operations is noteworthy since both performs RDMA read and write. In commit, iCheck makes sure that the data is ready to be transferred by performing an intra-node synchronisation at the beginning meanwhile during restart, an inter-node synchronisation occurs which leads to a large checkpoint restart time. The time taken for actual data transfer is similar to commit however, the explicit synchronisation adds the additional overhead. This synchronisation is essential to support automatic data redistribution, an extension under development in iCheck. Furthermore, the restart operation will only be performed once during the lifecycle of a non malleable application, while on the other hand the frequency of commit operations will be high. Nevertheless, increasing the number of agents can dramatically reduce the restart time as seen in the plot.

\subsubsection{Impact of dynamic agents in heat simulation}\label{subsec:dynamicagents}
%We can conclude from the above sections that checkpointing performance improves significantly in applications with a higher number of agents. This section examines whether this holds in the case of dynamically expanding the agents in an application. A 2D Jacobi heat simulation application, launched with 576 processes that checkpoint a total of 1.4GB, is used to evaluate on-the-fly agent adaptation. In this test scenario, \verb|icheck_probe_agents()| call will initiate the agent dynamism.

%The application is started with two agents, and we can observe in Figure~\ref{fig:ic_heat_dyn} that it took around .7 seconds to transfer each checkpoint. After a few seconds, we can see the performance improvement in data transfer. This improvement was the result of agent change performed by the controller. As seen in the figure, a performance improvement of up to 80\% is attained as new agents are added to the application. The overhead incurred by the application for a successful probe (agent change was initiated in the controller) was around 2.5 seconds (cost of four commits), while an unsuccessful probe (no change in agent configuration) took around 0.002 seconds. This overhead is negligible since we got double the performance improvement with each successful agent change. Hence, the cost for the probe can be nullified, and performance gain can be observed in the graph as more and more commits are performed. However, we need modelling and application-based heuristics to determine the ideal agent change that can immediately give the maximum performance to the application instead of step by step agent increase as seen in the figure. We can conclude that the iCheck functionality of dynamic agents provides significant performance improvement on-the-fly in our heat simulation application. 

%The application is started with two agents, and we can observe in Figure~\ref{fig:ic_heat_dyn} that it took around .7 seconds to transfer each checkpoint. After a few seconds, we can see the performance improvement in data transfer. This improvement was the result of agent change performed by the controller. As seen in the figure, a performance improvement of up to 80\% is attained as new agents are added to the application. The overhead incurred by the application for a successful agent change was around 2.5 seconds (cost of four commits). This overhead is negligible since we got double the performance improvement with each successful agent change. %Hence, the cost for the probe can be nullified, and performance gain can be observed in the graph as more and more commits are performed. 
%However, we need modelling and application-based heuristics to determine the ideal agent change that can immediately give the maximum performance to the application instead of step by step change as seen in the figure. %We can conclude that the iCheck functionality of dynamic agents provides significant performance improvement on-the-fly in our heat simulation application.

\subsubsection{Agent placement analysis with synthetic applications}\label{subsec:agent_placement}
%All of the above subsections primarily focussed on the effect of various number of agents on multiple applications. This subsection explores further and investigates the consequence of placing agents on iCheck nodes based on different strategies introduced in Section ~\ref{sec:iCheck}. 
%This subsection evaluates the placing of agents on iCheck nodes based on different strategies introduced in Section ~\ref{sec:iCheck}. In this analysis, we ran a synthetic application (say app A) in a continuous loop on two nodes (96 processes) with a single agent. Then, we ran an additional five synthetic applications (two nodes per application), placed the agents associated with these applications on different iCheck nodes, and studied their effect on app A's bandwidth with the ensuing agent placement strategies.
%1) Stacking: All the agents were placed in the same iCheck node as app A in this strategy.
%2) Bandwidth: Agents were placed on iCheck nodes with least activity (higher bandwidth will be available for data transfer).
%3) CP interval: Agents are placed in iCheck nodes that have a low checkpoint interval between applications.
%We can see from Figure ~\ref{fig:ic_synthetic_distribution} that these placement strategies can influence the performance of the application. For example, in the stacking strategy, the data transfer rate for checkpoints between the application and agents fluctuated between 3GB/s to 11.5GB/s. Meanwhile, in the strategies where agents are distributed among different iCheck nodes, the fluctuation is minimal. The strategy that always distributed the agents in iCheck nodes with least activity yielded the best performance (a bandwidth of 9.5GB/s to 11.5 GB/s) for our test app A. 

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=0.35\textwidth]{images/ic_synth_agent_placement.png}
%    \caption{Effect of agent placement}
%    \label{fig:ic_agent_placement}
%\end{figure}

\subsubsection{Horizontal scaling and agent placement analysis}\label{subsec:hs}
%In the above subsections, we showcase the dynamic placement of agents and dynamic change in agents during the application run. Apart from the dynamism offered to applications, iCheck itself is fully malleable and can grow or shrink based on the node availability. To fully utilize this ability, iCheck needs to be integrated with a malleable resource manager that can give/take nodes to/from the iCheck system based on the system status. Hence, a concrete evaluation of this feature is not yet possible and is beyond the scope of this work.

%iCheck is fully malleable and can grow or shrink based on the node availability. To fully utilize this ability, iCheck needs to be integrated with a malleable resource manager that can give/take nodes to/from the iCheck system based on the system status. Hence, a concrete evaluation of this feature is not yet possible and is beyond the scope of this work.
%However, we can demonstrate the ability of iCheck to scale its nodes horizontally by simulating a scenario were nodes are given to iCheck in predefined time intervals. Then we will launch the ls1 mardyn (on two nodes), LULESH(on two nodes), heat distribution (on four nodes), and synthetic (on four nodes) applications with a prescheduled agent distribution of one, two, four and four agents respectively in predetermined intervals. The agent placement strategy that gave best performance in Subsection~\ref{subsec:agent_placement} is used in this analysis.

%We can observe the results of the experiments in Figure ~\ref{fig:ic_scale} and ~\ref{fig:ic_scale_dist}. The former figure depicts the active iCheck nodes during a time interval, and the latter displays the agent to iCheck node placement during the same period. The increase in the iCheck nodes as seen in Figure ~\ref{fig:ic_scale} validates the ability of our system to scale as the resources (nodes) becomes available. Additionally, we can infer from the second Figure~\ref{fig:ic_scale_dist} that not only was iCheck able to scale horizontally but also used these new iCheck nodes for agent placement. Initially, ls1 mardyn was launched with a single agent, and it is placed in the only available node (See iCheck node 1 in Figure~\ref{fig:ic_scale_dist}). Later, we can see that a new node (iCheck node 2) was added at around the 40th second (See Figure~\ref{fig:ic_scale}). When LULESH was started, the two agents assigned to it were distributed among the iCheck node one and iCheck node two. We can observe it in Figure~\ref{fig:ic_scale_dist} (See 150th second).  

\subsection{Discussion on iCheck, malleability and beyond}\label{subsec:discussion}
%By having the horizontal scaling capability (demonstrated in subsection~\ref{subsec:hs}), iCheck brings the following two benefits to checkpointing in HPC. Firstly, there is no need to specify a dedicated set of nodes for checkpointing. The number and types of nodes allocated to checkpointing services can be varied on-the-fly by a resource manager. Secondly, as HPC is moving towards the cloud ~\cite{hpconcloud}, a dynamically scaling fault-tolerant system will benefit from a cost-based cloud model where it can expand or shrink its checkpointing nodes and agents based on the application demands and objectives.

%We can see (from subsection~\ref{subsec:dynamicagents}) that dynamically adding agents improves the checkpointing time, and placing the agents across different nodes can significantly improve the checkpointing bandwidth (subsection~\ref{subsec:agent_placement}). The malleability offered by iCheck enables combining these two functionalities whenever possible and creates a faster and more efficient checkpoint transfer mechanism.
 
%At present, HPC is going beyond homogeneous systems as more GPUs and accelerators are added to HPC systems~\cite{gpufpga,accel}. The design of iCheck support both homogeneous and heterogeneous systems. iCheck core can run out-of-the-box on the heterogeneous nodes of a cluster. The current implementation of the iCheck API that supports MPI and non-MPI applications can be further extended to support GPUDirect RDMA~\cite{gpurdma} to transfer data directly from GPUs to the iCheck core.

==> sections/library.tex <==
\section{iCheck Library}
\label{sec:library}
\subsection{API Design}

iCheck provides a minimalistic API for application-level coordinated checkpointing. A minimum of six iCheck API calls is needed for a successful C/R operation, of which two each for configuration, checkpoint, and restart. The configuration API call \verb|icheck_init()| registers the Application with the iCheck ecosystem while \verb|icheck_finalize()| will deregister it. \verb|icheck_add()| records the data, the type, and size to be checkpointed. The \verb|icheck_commit()| call will trigger the RDMA operations and transfers the checkpoint to the Agent. \verb|icheck_restart()|, and \verb|icheck_restore()| are used during the Application restart.

Additionally, iCheck provides special API calls to support dynamism and performance improvement. For example, \verb|icheck_probe_agents| will query the Controller for any change in the agent configuration. Based on the strategies defined in Section, the controller will respond to such queries either with more agents, fewer agents, or with a no-change response.

\subsection{Sample Application}

Pseudocode of a sample iCheck enabled application is in the Listing \ref{icheckapi}.\verb|icheck_init| requires the \verb|MPI_COMM_WORLD| communicator, application name as well as status.

\begin{minipage}{.469\textwidth}
\lstset{language=C++, basicstyle=\small,captionpos=b,caption={Pseudocode using iCheck API},label=icheckapi, keepspaces=true, stepnumber=1, firstnumber=1, numberfirstline=true}
\begin{lstlisting}[frame=single]
#include<icheck.h>
int main() {
    MPI_Init(NULL, NULL);
    float data[SIZE];
    icheck_init(argv[1], "sample", 
                MPI_COMM_WORLD, status);
    icheck_restart();
    icheck_add("DataArray", data, 
                    SIZE, ICHECK_FLOAT);
    /*Computation*/
    icheck_restore("DataArray",data,SIZE);
    for(i = 0; i<N; i++) {
        /* Perform operation on data[] */
        icheck_commit();
        /* Computation */
    }
    icheck_finalize();
    MPI_Finalize();
}
\end{lstlisting}
\end{minipage}\hfill

\subsection{UML Diagram}
